Distribution Aligning Refinery of Pseudo-label for Imbalanced Semi-supervised Learning

While semi-supervised learning (SSL) has proven to be a promising way for leveraging unlabeled data when labeled data is scarce, the existing SSL algorithms typically assume that training class distributions are balanced. However, these SSL algorithms trained under imbalanced class distributions can severely suffer when generalizing to a balanced testing criterion, since they utilize biased pseudo-labels of unlabeled data toward majority classes. To alleviate this issue, we formulate a convex optimization problem to softly refine the pseudo-labels generated from the biased model, and develop a simple algorithm, named Distribution Aligning Refinery of Pseudo-label (DARP) that solves it provably and efficiently. Under various class-imbalanced semi-supervised scenarios, we demonstrate the effectiveness of DARP and its compatibility with state-of-the-art SSL schemes.

==> Algs/Overall.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[h]
\caption{Current Algorithm}\label{alg:overall}
\begin{algorithmic}[1]
%\vspace{-0.04in}
\REQUIRE Labeled dataset $\mathcal{D}_{l}=\{(x^{(n)}_{l}, y^{(n)}_{l})\}_{n=1}^{N_{l}}$, unlabeled dataset $\mathcal{D}_{u}=\{x^{(n)}_{u}\}_{n=1}^{N_{u}}$ and validation dataset $\mathcal{D}_{v} = \{(x^{(n)}_{v},y^{(n)}_{v})\}_{n=1}^{N_{v}}$. Classifier $f_{\theta}(\cdot)$. Number of augmentations $M$. Sharpening temperature $T$. Unsupervised loss weight $\lambda_{u}$. Mixup parameter $\alpha$.  Hyper-parameter for distribution alignment $\beta$.
\vspace{0.05in}
\hrule
\vspace{0.05in}
\WHILE{$e < \text{MaxEpoch}$}
    \STATE $\Tilde{q}(y) \leftarrow \text{By Alg \ref{alg:estimation}} \text{~with~} \mathcal{D}_{u}, \mathcal{D}_{v} \text{~or~given}$
    \STATE $q_{\theta}(y) \leftarrow \frac{1}{N_u} \sum_{m=1}^{N_u} f_{\theta}(x^{(m)}_u)$
    \STATE $\Tilde{\mathcal{D}}_{u} \leftarrow \text{By Alg \ref{alg:pseudo}} \text{~with~} \mathcal{D}_{u}, \Tilde{q}(y)$
    \FOR{$\text{iter}=1$ {\bfseries to} $\text{num\textunderscore iters}$}
        \STATE Draw a mini-batch $\mathcal{X} = \{ (x_{l}^{(b)}, y_{l}^{(b)})\}^{B}_{b=1} \sim \mathcal{D}_{l}$
        \STATE Draw a mini-batch $\hat{\mathcal{U}} = \{ (x_{u}^{(b)}, \hat{y}_{u}^{(b)}) \}^{B}_{b=1} \sim \Tilde{\mathcal{D}}_{u}$
        \FOR{$b=1$ {\bfseries to} $B$}
            \STATE $q_b = \text{Augment \& Sharp}(x_{u}^{(b)}, f_{\theta}, M, T)$
            \STATE \textcolor{blue}{ $\rhd$ $q_b$ is the pseudo label from MixMatch}
            \STATE $\hat{y}_{u}^{(b)} \leftarrow \text{Normalize}\big( q_b \times ( \beta \cdot \frac{\Tilde{q}(y)}{q_{\theta}(y)} + (1 - \beta) \cdot \frac{\hat{y}_{u}^{b}}{q_b}) \big)$
        \ENDFOR
        \STATE $\mathcal{L}_{\mathcal{X}}, \mathcal{L}_{\mathcal{U}} = \text{MixMatch}(\mathcal{X}, \hat{\mathcal{U}}, \alpha)$
        \STATE $\mathcal{L} = \mathcal{L}_{\mathcal{X}} + \lambda_{u} \mathcal{L}_{\mathcal{U}}$
        \STATE $\theta \leftarrow \theta - \eta \cdot \nabla \mathcal{L}$
    \ENDFOR
\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> Algs/darp_backup.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[t]
\caption{$\mathtt{DARP}$: Distribution aligning refinery of pseudo-label}\label{alg:pseudo}
\begin{algorithmic}[1]
%\vspace{-0.04in}
\REQUIRE Unlabeled data $\{x^{\tt unlabeled}_{m}\}_{m=1}^M$, pseudo-labels $\{\hat y_m^{\tt unlabeled}\}_{m=1}^M$, sample-wise weights $\{w_m\}_{m=1}^M$, true class distribution $\{M_{k}\}_{k=1}^K$, number of classes $K$, number of iterations $T$, hyper-parameter for removing noisy pseudo-label entries $\delta$.
\ENSURE Refined pseudo-labels $\hat y_{m}^{\tt DARP}$ 
\vspace{0.05in}
\hrule
\vspace{0.05in}
%\STATE $w_m \leftarrow 1 ~/~ \sum_{k=1}^{K} - \hat y_{m}^{\tt unlabeled}(k) \log \hat y_{m}^{\tt unlabeled}(k) ~\forall m$
\FOR{$k=1$ {\bfseries to} $K$}
    \STATE $\{\hat{m}_{1}, \dots, \hat{m}_{M}\} \leftarrow \mathtt{Sort}\big( \{ y_m^{\tt unlabeled}(k)\,|\,\forall m\}\big)$ \\  %\textcolor{black}{// Sort: outputs sorted indices in descending order}
    \STATE $\mathcal{U}_{k} = \{x^{\tt unlabeled}_{\hat{m}_{1}}, \dots, x^{\tt unlabeled}_{\hat{m}_{\hat{\delta}}} \}$,~$\hat{\delta} = \lfloor \delta \cdot M_{k} \rfloor$
\ENDFOR
\STATE $\hat y_{m}^{\tt unlabeled}(k) \leftarrow \begin{cases} \hat y_{m}^{\tt unlabeled}(k) & \text{if}~ x_{m}^{\tt unlabeled} \in \mathcal{U}_{k} \\  \qquad~~ 0 & \text{otherwise} \end{cases},~ \alpha_{m}^{0} = \beta_{k}^{0} = 1 \quad \forall m,k$
\STATE $\hat{y}^{\tt DARP}_{m}(k) \leftarrow\mathtt{DualCoordinateAscent}
\left(\{\hat y_m^{\tt unlabeled}\}_{m=1}^M,  \{w_m\}_{m=1}^M, \{M_{k}\}_{k=1}^K, T\right)$

\iffalse
\FOR{$t=1$ {\bfseries to} $T$}
    \IF{$t$ is odd or $t=T$} \vspace{0.02in}
    \STATE $X^{t}_{m} \leftarrow 1~/~\sum_{k=1}^{K} \hat y_{m}^{0}(k) (Y^{t-1}_{k})^{\frac{1}{w_m}}, ~~ Y^{t}_{k} \leftarrow Y^{t-1}_{k} \quad \forall m,k$ 
    \ELSE
    \STATE $Y^{t}_{k} \leftarrow \text{Newton-Raphson}(\sum_{m=1}^{M} \hat y_m^{0}(k) X_{m}^{t-1}(Y_{k}^{t})^{\frac{1}{w_m}} - M_{k}), ~~ X^{t}_{k} \leftarrow X^{t-1}_{k} \quad \forall m,k$  
    \ENDIF
\ENDFOR
\STATE $\hat{y}^{\tt DARP}_{m}(k) \leftarrow \hat y_m^{0}(k) X^{T}_{m} (Y^{T}_{k})^{\frac{1}{w_m}} \quad \forall m,k$
\fi

\end{algorithmic}
\end{algorithm}
%\vspace{-0.1in}

% ICML version
\iffalse
\begin{algorithm}[t]
\caption{Distribution Aligning Refinery of Pseudo-label (DARP)}\label{alg:pseudo}
\begin{algorithmic}[1]
%\vspace{-0.04in}
\REQUIRE unlabeled data $\{x^{\tt unlabeled}_{m}\}$, pseudo-labels $\{\hat y_m^{\tt unlabeled}\}$, number of classes $K$, true class distribution $\{M_{k}\}$, number of iterations $T$. 
\ENSURE Refined pseudo-labels $\hat y_{m}^{\tt DARP}$ 
\vspace{0.05in}
\hrule
\vspace{0.05in}
\FOR{$k=1$ {\bfseries to} $K$}
    \STATE $\{\hat{m}_{1}, \dots, \hat{m}_{M}\} \leftarrow \text{Sort}\big( \{ y_m^{\tt unlabeled}(k)\,|\,\forall m\}\big)$ \\  %\textcolor{black}{// Sort: outputs sorted indices in descending order}
    \STATE $\mathcal{U}_{k} = \{x^{\tt unlabeled}_{\hat{m}_{1}}, \dots, x^{\tt unlabeled}_{\hat{m}_{\hat{\delta}}} \}$,~$\hat{\delta} = \lfloor \delta \cdot M_{k} \rfloor$
\ENDFOR
\STATE $\hat y_{m}^{0}(k) \leftarrow \begin{cases} \hat y_{m}^{\tt unlabeled}(k) & \text{if}~ x_{m}^{\tt unlabeled} \in \mathcal{U}_{k} \\  \qquad~~ 0 & \text{otherwise} \end{cases}$

\FOR{$t=1$ {\bfseries to} $T$}
    \IF{$t$ is odd}
    \STATE $\hat{y}^{t}_{m}(k) \leftarrow M_{k} \cdot \hat{y}^{t-1}_{m}(k) ~/~ \sum_{m^\prime=1}^{M} \hat{y}^{t-1}_{m^\prime}(k),~\forall m,k$
    \ELSE
    \STATE $\hat{y}^{t}_{m}(k) \leftarrow \hat{y}^{t-1}_{m}(k) ~/~ \sum_{k^\prime=1}^{K} \hat{y}^{t-1}_{m}(k^\prime),~\forall m,k$
    \ENDIF
\ENDFOR
\STATE $\hat{y}^{\tt DARP}_{m}\leftarrow \hat{y}^{T}_{m},\quad\forall m$
\end{algorithmic}
\end{algorithm}
\fi

==> Algs/estimation.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[h]
\caption{Estimation of $q(y)$}\label{alg:estimation}
\begin{algorithmic}[1]
%\vspace{-0.04in}
\REQUIRE Unlabeled dataset $\mathcal{D}_{u}=\{x^{(m)}_{u}\}_{m=1}^{N_{u}}$ and validation dataset $\mathcal{D}_{v} = \{(x^{(n)}_{v},y^{(n)}_{v})\}_{n=1}^{N_{v}}$. Classifier $f_{\theta}(\cdot)$. 
\ENSURE Estimated marginal distribution $\Tilde{q}(y)$
\vspace{0.05in}
\hrule
\vspace{0.05in}
\STATE Initialize $C \in \mathbb{R}^{K \times K}$ with zeros
\FOR{$k=1$ {\bfseries to} $K$}
    \STATE $n_k = 0$
    \FOR{$(x^{(n)}_v,y^{(n)}_v) \in \mathcal{D}_{v}$ such that $y^{(n)}_v=k$}
        \STATE $C_{\cdot,k} \leftarrow C_{\cdot,k} + f_{\theta}(x^{(n)}_v),~ n_c \leftarrow n_c + 1$
    \ENDFOR    
    \STATE $C_{\cdot,k} \leftarrow C_{\cdot,k} / n_c$
\ENDFOR
\STATE $q_{\theta}(y) = \sum_{m=1}^{N_{u}} f_{\theta}(x^{(m)}_{u}) / N_{u}$
\STATE $\Tilde{q}(y) = \sum_{\Tilde{y}} C^{-1}(y,\Tilde{y}) q_{\theta}(\Tilde{y})$
\end{algorithmic}
\end{algorithm}

==> Algs/pseudo.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[ht]
\caption{Distributionally Aligned Pseudo Labeling}\label{alg:pseudo2}
\begin{algorithmic}[1]
%\vspace{-0.04in}
\REQUIRE Unlabeled data $\mathcal{D}_{u}=\{u_{m}\}_{m=1}^{M}$ with class distribution $q(y)$. Classifier $f(\cdot)$. 
\ENSURE Pseudo-labeled data $\Tilde{\mathcal{D}}_{u}=\{(u_{m},\tilde{y}_{u,m})\}_{m=1}^{M}$
\vspace{0.05in}
\hrule
\vspace{0.05in}
\STATE Initialize $\Tilde{\mathcal{D}}_{u} \leftarrow \text{\o}, \mathcal{M} =\{1,\dots,M\}$
\FOR{$k=K$ {\bfseries to} $1$}
    \STATE $[\Tilde{m}_{1}, \dots, \Tilde{m}_{|\mathcal{M}|}] \leftarrow \text{Sort}\big( \{ f_{k}(u_{m}) | m \in \mathcal{M} \}\big)$
    \STATE \textcolor{blue}{$\rhd$ Sort: outputs sorted indices in descending order}
    \STATE $\Tilde{\mathcal{M}}_{k} = [\Tilde{m}_{1}, \dots, \Tilde{m}_{N_{k}}]$, $N_k= \lfloor q(k) \cdot M \rfloor$
    \STATE $\Tilde{\mathcal{D}}_{u} \leftarrow \Tilde{\mathcal{D}}_{u} \cup \{(u_{\tilde{m}}, k)|\Tilde{m} \in \Tilde{\mathcal{M}}_{k}\}$
    \STATE $\mathcal{M} \leftarrow \mathcal{M} \setminus \Tilde{\mathcal{M}}_{k}$
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> Imbalanced Semi-supervised Learning Arxiv (3)/Algs/Overall.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[h]
\caption{Current Algorithm}\label{alg:overall}
\begin{algorithmic}[1]
%\vspace{-0.04in}
\REQUIRE Labeled dataset $\mathcal{D}_{l}=\{(x^{(n)}_{l}, y^{(n)}_{l})\}_{n=1}^{N_{l}}$, unlabeled dataset $\mathcal{D}_{u}=\{x^{(n)}_{u}\}_{n=1}^{N_{u}}$ and validation dataset $\mathcal{D}_{v} = \{(x^{(n)}_{v},y^{(n)}_{v})\}_{n=1}^{N_{v}}$. Classifier $f_{\theta}(\cdot)$. Number of augmentations $M$. Sharpening temperature $T$. Unsupervised loss weight $\lambda_{u}$. Mixup parameter $\alpha$.  Hyper-parameter for distribution alignment $\beta$.
\vspace{0.05in}
\hrule
\vspace{0.05in}
\WHILE{$e < \text{MaxEpoch}$}
    \STATE $\Tilde{q}(y) \leftarrow \text{By Alg \ref{alg:estimation}} \text{~with~} \mathcal{D}_{u}, \mathcal{D}_{v} \text{~or~given}$
    \STATE $q_{\theta}(y) \leftarrow \frac{1}{N_u} \sum_{m=1}^{N_u} f_{\theta}(x^{(m)}_u)$
    \STATE $\Tilde{\mathcal{D}}_{u} \leftarrow \text{By Alg \ref{alg:pseudo}} \text{~with~} \mathcal{D}_{u}, \Tilde{q}(y)$
    \FOR{$\text{iter}=1$ {\bfseries to} $\text{num\textunderscore iters}$}
        \STATE Draw a mini-batch $\mathcal{X} = \{ (x_{l}^{(b)}, y_{l}^{(b)})\}^{B}_{b=1} \sim \mathcal{D}_{l}$
        \STATE Draw a mini-batch $\hat{\mathcal{U}} = \{ (x_{u}^{(b)}, \hat{y}_{u}^{(b)}) \}^{B}_{b=1} \sim \Tilde{\mathcal{D}}_{u}$
        \FOR{$b=1$ {\bfseries to} $B$}
            \STATE $q_b = \text{Augment \& Sharp}(x_{u}^{(b)}, f_{\theta}, M, T)$
            \STATE \textcolor{blue}{ $\rhd$ $q_b$ is the pseudo label from MixMatch}
            \STATE $\hat{y}_{u}^{(b)} \leftarrow \text{Normalize}\big( q_b \times ( \beta \cdot \frac{\Tilde{q}(y)}{q_{\theta}(y)} + (1 - \beta) \cdot \frac{\hat{y}_{u}^{b}}{q_b}) \big)$
        \ENDFOR
        \STATE $\mathcal{L}_{\mathcal{X}}, \mathcal{L}_{\mathcal{U}} = \text{MixMatch}(\mathcal{X}, \hat{\mathcal{U}}, \alpha)$
        \STATE $\mathcal{L} = \mathcal{L}_{\mathcal{X}} + \lambda_{u} \mathcal{L}_{\mathcal{U}}$
        \STATE $\theta \leftarrow \theta - \eta \cdot \nabla \mathcal{L}$
    \ENDFOR
\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> Imbalanced Semi-supervised Learning Arxiv (3)/Algs/darp.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[t]
\caption{$\mathtt{DARP}$: Distribution aligning refinery of pseudo-label}\label{alg:pseudo}
\begin{algorithmic}[1]
%\vspace{-0.04in}
\REQUIRE Unlabeled data $\{x^{\tt unlabeled}_{m}\}_{m=1}^M$, pseudo-labels $\{\hat y_m^{\tt unlabeled}\}_{m=1}^M$, sample-wise weights $\{w_m\}_{m=1}^M$, true class distribution $\{M_{k}\}_{k=1}^K$, number of classes $K$, number of iterations $T$, hyper-parameter for removing noisy pseudo-label entries $\delta$.
\ENSURE Refined pseudo-labels $\hat y_{m}^{\tt DARP}$ 
\vspace{0.05in}
\hrule
\vspace{0.05in}
%\STATE $w_m \leftarrow 1 ~/~ \sum_{k=1}^{K} - \hat y_{m}^{\tt unlabeled}(k) \log \hat y_{m}^{\tt unlabeled}(k) ~\forall m$
\FOR{$k=1$ {\bfseries to} $K$}
    \STATE $\{\hat{m}_{1}, \dots, \hat{m}_{M}\} \leftarrow \mathtt{Sort}\big( \{ y_m^{\tt unlabeled}(k)\,|\,\forall m\}\big)$ \\  %\textcolor{black}{// Sort: outputs sorted indices in descending order}
    \STATE $\mathcal{U}_{k} = \{x^{\tt unlabeled}_{\hat{m}_{1}}, \dots, x^{\tt unlabeled}_{\hat{m}_{\hat{\delta}}} \}$,~$\hat{\delta} = \lfloor \delta \cdot M_{k} \rfloor$
\ENDFOR
\STATE $\hat y_{m}^{\tt unlabeled}(k) \leftarrow \begin{cases} \hat y_{m}^{\tt unlabeled}(k) & \text{if}~ x_{m}^{\tt unlabeled} \in \mathcal{U}_{k} \\  \qquad~~ 0 & \text{otherwise} \end{cases},~ \alpha_{m}^{0} = \beta_{k}^{0} = 1 \quad \forall m,k$
\STATE $\hat{y}^{\tt DARP}_{m}(k) \leftarrow\mathtt{DualCoordinateAscent}
\left(\{\hat y_m^{\tt unlabeled}\}_{m=1}^M,  \{w_m\}_{m=1}^M, \{M_{k}\}_{k=1}^K, T\right)$

\end{algorithmic}
\end{algorithm}

==> Imbalanced Semi-supervised Learning Arxiv (3)/Algs/darp_backup.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[t]
\caption{$\mathtt{DARP}$: Distribution aligning refinery of pseudo-label}\label{alg:pseudo}
\begin{algorithmic}[1]
%\vspace{-0.04in}
\REQUIRE Unlabeled data $\{x^{\tt unlabeled}_{m}\}_{m=1}^M$, pseudo-labels $\{\hat y_m^{\tt unlabeled}\}_{m=1}^M$, sample-wise weights $\{w_m\}_{m=1}^M$, true class distribution $\{M_{k}\}_{k=1}^K$, number of classes $K$, number of iterations $T$, hyper-parameter for removing noisy pseudo-label entries $\delta$.
\ENSURE Refined pseudo-labels $\hat y_{m}^{\tt DARP}$ 
\vspace{0.05in}
\hrule
\vspace{0.05in}
%\STATE $w_m \leftarrow 1 ~/~ \sum_{k=1}^{K} - \hat y_{m}^{\tt unlabeled}(k) \log \hat y_{m}^{\tt unlabeled}(k) ~\forall m$
\FOR{$k=1$ {\bfseries to} $K$}
    \STATE $\{\hat{m}_{1}, \dots, \hat{m}_{M}\} \leftarrow \mathtt{Sort}\big( \{ y_m^{\tt unlabeled}(k)\,|\,\forall m\}\big)$ \\  %\textcolor{black}{// Sort: outputs sorted indices in descending order}
    \STATE $\mathcal{U}_{k} = \{x^{\tt unlabeled}_{\hat{m}_{1}}, \dots, x^{\tt unlabeled}_{\hat{m}_{\hat{\delta}}} \}$,~$\hat{\delta} = \lfloor \delta \cdot M_{k} \rfloor$
\ENDFOR
\STATE $\hat y_{m}^{\tt unlabeled}(k) \leftarrow \begin{cases} \hat y_{m}^{\tt unlabeled}(k) & \text{if}~ x_{m}^{\tt unlabeled} \in \mathcal{U}_{k} \\  \qquad~~ 0 & \text{otherwise} \end{cases},~ \alpha_{m}^{0} = \beta_{k}^{0} = 1 \quad \forall m,k$
\STATE $\hat{y}^{\tt DARP}_{m}(k) \leftarrow\mathtt{DualCoordinateAscent}
\left(\{\hat y_m^{\tt unlabeled}\}_{m=1}^M,  \{w_m\}_{m=1}^M, \{M_{k}\}_{k=1}^K, T\right)$

\iffalse
\FOR{$t=1$ {\bfseries to} $T$}
    \IF{$t$ is odd or $t=T$} \vspace{0.02in}
    \STATE $X^{t}_{m} \leftarrow 1~/~\sum_{k=1}^{K} \hat y_{m}^{0}(k) (Y^{t-1}_{k})^{\frac{1}{w_m}}, ~~ Y^{t}_{k} \leftarrow Y^{t-1}_{k} \quad \forall m,k$ 
    \ELSE
    \STATE $Y^{t}_{k} \leftarrow \text{Newton-Raphson}(\sum_{m=1}^{M} \hat y_m^{0}(k) X_{m}^{t-1}(Y_{k}^{t})^{\frac{1}{w_m}} - M_{k}), ~~ X^{t}_{k} \leftarrow X^{t-1}_{k} \quad \forall m,k$  
    \ENDIF
\ENDFOR
\STATE $\hat{y}^{\tt DARP}_{m}(k) \leftarrow \hat y_m^{0}(k) X^{T}_{m} (Y^{T}_{k})^{\frac{1}{w_m}} \quad \forall m,k$
\fi

\end{algorithmic}
\end{algorithm}
%\vspace{-0.1in}

% ICML version
\iffalse
\begin{algorithm}[t]
\caption{Distribution Aligning Refinery of Pseudo-label (DARP)}\label{alg:pseudo}
\begin{algorithmic}[1]
%\vspace{-0.04in}
\REQUIRE unlabeled data $\{x^{\tt unlabeled}_{m}\}$, pseudo-labels $\{\hat y_m^{\tt unlabeled}\}$, number of classes $K$, true class distribution $\{M_{k}\}$, number of iterations $T$. 
\ENSURE Refined pseudo-labels $\hat y_{m}^{\tt DARP}$ 
\vspace{0.05in}
\hrule
\vspace{0.05in}
\FOR{$k=1$ {\bfseries to} $K$}
    \STATE $\{\hat{m}_{1}, \dots, \hat{m}_{M}\} \leftarrow \text{Sort}\big( \{ y_m^{\tt unlabeled}(k)\,|\,\forall m\}\big)$ \\  %\textcolor{black}{// Sort: outputs sorted indices in descending order}
    \STATE $\mathcal{U}_{k} = \{x^{\tt unlabeled}_{\hat{m}_{1}}, \dots, x^{\tt unlabeled}_{\hat{m}_{\hat{\delta}}} \}$,~$\hat{\delta} = \lfloor \delta \cdot M_{k} \rfloor$
\ENDFOR
\STATE $\hat y_{m}^{0}(k) \leftarrow \begin{cases} \hat y_{m}^{\tt unlabeled}(k) & \text{if}~ x_{m}^{\tt unlabeled} \in \mathcal{U}_{k} \\  \qquad~~ 0 & \text{otherwise} \end{cases}$

\FOR{$t=1$ {\bfseries to} $T$}
    \IF{$t$ is odd}
    \STATE $\hat{y}^{t}_{m}(k) \leftarrow M_{k} \cdot \hat{y}^{t-1}_{m}(k) ~/~ \sum_{m^\prime=1}^{M} \hat{y}^{t-1}_{m^\prime}(k),~\forall m,k$
    \ELSE
    \STATE $\hat{y}^{t}_{m}(k) \leftarrow \hat{y}^{t-1}_{m}(k) ~/~ \sum_{k^\prime=1}^{K} \hat{y}^{t-1}_{m}(k^\prime),~\forall m,k$
    \ENDIF
\ENDFOR
\STATE $\hat{y}^{\tt DARP}_{m}\leftarrow \hat{y}^{T}_{m},\quad\forall m$
\end{algorithmic}
\end{algorithm}
\fi

==> Imbalanced Semi-supervised Learning Arxiv (3)/Algs/estimation.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[h]
\caption{Estimation of $q(y)$}\label{alg:estimation}
\begin{algorithmic}[1]
%\vspace{-0.04in}
\REQUIRE Unlabeled dataset $\mathcal{D}_{u}=\{x^{(m)}_{u}\}_{m=1}^{N_{u}}$ and validation dataset $\mathcal{D}_{v} = \{(x^{(n)}_{v},y^{(n)}_{v})\}_{n=1}^{N_{v}}$. Classifier $f_{\theta}(\cdot)$. 
\ENSURE Estimated marginal distribution $\Tilde{q}(y)$
\vspace{0.05in}
\hrule
\vspace{0.05in}
\STATE Initialize $C \in \mathbb{R}^{K \times K}$ with zeros
\FOR{$k=1$ {\bfseries to} $K$}
    \STATE $n_k = 0$
    \FOR{$(x^{(n)}_v,y^{(n)}_v) \in \mathcal{D}_{v}$ such that $y^{(n)}_v=k$}
        \STATE $C_{\cdot,k} \leftarrow C_{\cdot,k} + f_{\theta}(x^{(n)}_v),~ n_c \leftarrow n_c + 1$
    \ENDFOR    
    \STATE $C_{\cdot,k} \leftarrow C_{\cdot,k} / n_c$
\ENDFOR
\STATE $q_{\theta}(y) = \sum_{m=1}^{N_{u}} f_{\theta}(x^{(m)}_{u}) / N_{u}$
\STATE $\Tilde{q}(y) = \sum_{\Tilde{y}} C^{-1}(y,\Tilde{y}) q_{\theta}(\Tilde{y})$
\end{algorithmic}
\end{algorithm}

==> Imbalanced Semi-supervised Learning Arxiv (3)/Algs/pseudo.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[ht]
\caption{Distributionally Aligned Pseudo Labeling}\label{alg:pseudo2}
\begin{algorithmic}[1]
%\vspace{-0.04in}
\REQUIRE Unlabeled data $\mathcal{D}_{u}=\{u_{m}\}_{m=1}^{M}$ with class distribution $q(y)$. Classifier $f(\cdot)$. 
\ENSURE Pseudo-labeled data $\Tilde{\mathcal{D}}_{u}=\{(u_{m},\tilde{y}_{u,m})\}_{m=1}^{M}$
\vspace{0.05in}
\hrule
\vspace{0.05in}
\STATE Initialize $\Tilde{\mathcal{D}}_{u} \leftarrow \text{\o}, \mathcal{M} =\{1,\dots,M\}$
\FOR{$k=K$ {\bfseries to} $1$}
    \STATE $[\Tilde{m}_{1}, \dots, \Tilde{m}_{|\mathcal{M}|}] \leftarrow \text{Sort}\big( \{ f_{k}(u_{m}) | m \in \mathcal{M} \}\big)$
    \STATE \textcolor{blue}{$\rhd$ Sort: outputs sorted indices in descending order}
    \STATE $\Tilde{\mathcal{M}}_{k} = [\Tilde{m}_{1}, \dots, \Tilde{m}_{N_{k}}]$, $N_k= \lfloor q(k) \cdot M \rfloor$
    \STATE $\Tilde{\mathcal{D}}_{u} \leftarrow \Tilde{\mathcal{D}}_{u} \cup \{(u_{\tilde{m}}, k)|\Tilde{m} \in \Tilde{\mathcal{M}}_{k}\}$
    \STATE $\mathcal{M} \leftarrow \mathcal{M} \setminus \Tilde{\mathcal{M}}_{k}$
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> Imbalanced Semi-supervised Learning Arxiv (3)/table/Table1.tex <==
\begin{table*}[t]
	\begin{center}
	\caption{Comparison of classification performance (bACC/GM) on CIFAR-10 under three different class-imbalance ratio $\gamma=\gamma_l=\gamma_u$. SSL denotes semi-supervised learning and RB denotes re-balancing. The numbers in brackets below the gray rows are relative test error gains from DARP, compared to applied baseline SSL algorithms, respectively. The best results are indicated in bold.
    }
	\label{table:cifar_main}
    \begin{adjustbox}{width=0.85\linewidth}
	\begin{tabular}{cccccc}
		\toprule
		\multicolumn{3}{c}{}   & \multicolumn{3}{c}{CIFAR-10 ($\gamma=\gamma_{l}=\gamma_{u}$)} \\
        \cmidrule(r){4-6}
        \vspace{0.15in}
		\multirow{2}{*}{Algorithm}       &
		\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} SSL \end{tabular}} &   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} RB \end{tabular}}
		              & \multirow{2}{*}{$\gamma=50$}  
		              & \multirow{2}{*}{$\gamma=100$}
		              & \multirow{2}{*}{$\gamma=150$} \\ \midrule
		Vanilla       & - & - 
		              & {65.2\ms{0.05}} / {61.1\ms{0.09}} 
		              & {58.8\ms{0.13}} / {51.0\ms{0.11}} 
		              & {55.6\ms{0.43}} / {44.0\ms{0.98}} 
		               \\\midrule 
	    Re-sampling \cite{japkowicz2000class}   & - & \checkmark  
		              & {64.3\ms{0.48}} / {60.6\ms{0.67}}
		              & {55.8\ms{0.47}} / {45.1\ms{0.30}}
		              & {52.2\ms{0.05}} / {38.2\ms{1.49}}
		              \\ 
	    LDAM-DRW \cite{cao2019learning}     & - & \checkmark 
		              & {68.9\ms{0.07}} / {67.0\ms{0.08}}
		              & {62.8\ms{0.17}} / {58.9\ms{0.60}} 
		              & {57.9\ms{0.20}} / {50.4\ms{0.30}}
		              \\ 
		cRT \cite{kang2019decoupling}          & - & \checkmark  
		              & {67.8\ms{0.13}} / {66.3\ms{0.15}} 
		              & {63.2\ms{0.45}} / {59.9\ms{0.40}} 
		              & {59.3\ms{0.10}} / {54.6\ms{0.72}}
		               \\ \midrule
		VAT \cite{miyato2018virtual}          &  \checkmark & -  
		              & {70.6\ms{0.29}} / {67.8\ms{0.19}} 
		              & {62.6\ms{0.40}} / {55.1\ms{0.56}} 
		              & {57.9\ms{0.42}} / {46.3\ms{0.47}}
		               \\ 
		Mean-Teacher \cite{tarvainen2017mean} &  \checkmark & -  
		              & {68.8\ms{1.05}} / {64.9\ms{1.53}} 
		              & {60.9\ms{0.33}} / {52.8\ms{0.81}} 
		              & {54.5\ms{0.22}} / {39.8\ms{0.73}}
		               \\ 
		MixMatch \cite{berthelot2019mixmatch}     &  \checkmark & - 
		              & {73.2\ms{0.56}} / {68.9\ms{1.15}}
		              & {64.8\ms{0.28}} / {49.0\ms{2.05}}
		              & {62.5\ms{0.31}} / {42.5\ms{1.68}}
		                \\
	\rowcolor{Gray}	 MixMatch + DARP             
	                  & \checkmark & - 
		              & {75.2\ms{0.47}} / {72.8\ms{0.63}}
		              & {67.9\ms{0.14}} / {61.2\ms{0.15}}
		              & {65.8\ms{0.52}} / {56.5\ms{2.08}} 
		              \\
		              & &   
		              & (-7.41\% / -12.6\%) 
		              & (-8.77\% / -23.8\%) 
		              & (-8.69\% / -24.4\%) 
		              \\
	    ReMixMatch \cite{berthelot2019remixmatch}   & \checkmark & - 
		              & {81.5\ms{0.26}} / {80.2\ms{0.32}} 
		              & {73.8\ms{0.38}} / {69.5\ms{0.84}} 
		              & {69.9\ms{0.47}} / {62.5\ms{0.35}}
		               \\
	\rowcolor{Gray} ReMixMatch + DARP
	                  & \checkmark & -
		              & {\textbf{82.1}\ms{0.14}} / {{80.8}\ms{0.09}}  
		              & {\textbf{75.8}\ms{0.09}} / {{72.6}\ms{0.24}} 
		              & {\textbf{71.0}\ms{0.27}} / {{64.5}\ms{0.68}} \\ 
		              & &   
		              & (-3.45\% / -3.52\%) 
		              & (-7.84\% / -10.2\%) 
		              & (-3.60\% / -5.19\%)  
		               \\
		FixMatch \cite{sohn2020fixmatch}     &  \checkmark & - 
		              & {79.2\ms{0.33}} / {77.8\ms{0.36}}
		              & {71.5\ms{0.72}} / {66.8\ms{1.51}}
		              & {68.4\ms{0.15}} / {59.9\ms{0.43}}
		               \\
	\rowcolor{Gray} FixMatch + DARP
	                  & \checkmark & - 
		              & {81.8\ms{0.24}} / {\textbf{80.9}\ms{0.28}}
		              & {75.5\ms{0.05}} / {\textbf{73.0}\ms{0.09}}
		              & {70.4\ms{0.25}} / {\textbf{64.9}\ms{0.17}} \\ 
		              & &   
		              & (-12.9\% / -14.1\%) 
		              & (-14.0\% / -18.8\%) 
		              & (-22.4\% / -20.3\%) 
		               \\\bottomrule
	\end{tabular}
    \end{adjustbox}
    \end{center}
    \vspace{-0.05in}
\end{table*}

==> Imbalanced Semi-supervised Learning Arxiv (3)/table/Table2.tex <==
\begin{table*}[t]
	\begin{center}
    \caption{Comparison of classification performance (bACC/GM) on CIFAR-10 under four different class-imbalance ratio $\gamma_u$ with $\gamma_l=100$. SSL denotes semi-supervised learning and RB denotes re-balancing. The numbers in brackets below the gray rows are relative test error gains from DARP, compared to applied baseline SSL algorithms, respectively. The best results are indicated in bold.}
    \label{table:shuffled}
    \begin{adjustbox}{width=1\linewidth}
	\begin{tabular}{ccccccc}
		\toprule
		\multicolumn{3}{c}{}   & \multicolumn{4}{c}{CIFAR-10 ($\gamma_{l}=100$)}  \\
        \cmidrule(r){4-7}  
        \vspace{0.15in}
        \multirow{2}{*}{Algorithm}   &  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} SSL \end{tabular}} &   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} RB \end{tabular}}    
		              & \multirow{2}{*}{$\gamma_{u}=1$}
		              & \multirow{2}{*}{$\gamma_{u}=50$} 
		              & \multirow{2}{*}{$\gamma_{u}=150$}
		              & \multirow{2}{*}{$\gamma_{u}=100 ~(\text{reversed})$}
		              \\\midrule
		Vanilla       & - & -  
		              & {58.8\ms{0.13}} / {51.0\ms{0.11}} 
		              & {58.8\ms{0.13}} / {51.0\ms{0.11}} 
		              & {58.8\ms{0.13}} / {51.0\ms{0.11}}~$\arrvline$
		              & {58.8\ms{0.13}} / {51.0\ms{0.11}} 
		               \\\midrule 
	    Re-sampling \cite{japkowicz2000class}  &  - & \checkmark  
		              & {55.8\ms{0.47}} / {45.1\ms{0.30}}
		              & {55.8\ms{0.47}} / {45.1\ms{0.30}} 
		              & {55.8\ms{0.47}} / {45.1\ms{0.30}}~$\arrvline$
		              & {55.8\ms{0.47}} / {45.1\ms{0.30}}
		               \\ 
	    LDAM-DRW \cite{cao2019learning}     &  - & \checkmark 
		              & {62.8\ms{0.17}} / {58.9\ms{0.60}} 
		              & {62.8\ms{0.17}} / {58.9\ms{0.60}}
		              & {62.8\ms{0.17}} / {58.9\ms{0.60}}~$\arrvline$
		              & {62.8\ms{0.17}} / {58.9\ms{0.60}}
		               \\ 
		cRT \cite{kang2019decoupling}          &  - & \checkmark  
		              & {63.2\ms{0.45}} / {59.9\ms{0.40}} 
		              & {63.2\ms{0.45}} / {59.9\ms{0.40}}
		              & {63.2\ms{0.45}} / {59.9\ms{0.40}}~$\arrvline$
		              & {63.2\ms{0.45}} / {59.9\ms{0.40}}
		               \\ \midrule
		VAT \cite{miyato2018virtual}           &  \checkmark & -  
		              & {65.2\ms{0.12}} / {59.5\ms{0.26}}
		              & {64.0\ms{0.31}} / {57.3\ms{0.66}}
		              & {62.8\ms{0.19}} / {55.1\ms{0.70}}~$\arrvline$
		              & {59.4\ms{0.36}} / {50.6\ms{0.61}}
		               \\ 
		Mean-Teacher \cite{tarvainen2017mean}  &  \checkmark & -  
		              & {73.9\ms{1.19}} / {71.7\ms{1.42}}
		              & {61.2\ms{0.51}} / {53.5\ms{0.84}}
		              & {59.7\ms{0.50}} / {50.0\ms{1.61}}~$\arrvline$
		              & {61.0\ms{0.82}} / {56.4\ms{1.64}}
		              \\ 
		MixMatch \cite{berthelot2019mixmatch}     &  \checkmark & - 
		              & {41.5\ms{0.76}} / {12.0\ms{1.34}}
		              & {64.1\ms{0.58}} / {48.3\ms{0.70}}
		              & {65.5\ms{0.64}} / {51.1\ms{2.41}}~$\arrvline$ 
		              & {47.9\ms{0.09}} / {20.5\ms{0.85}}
		              \\
		              \rowcolor{Gray} MixMatch + DARP  &  \checkmark & - 
		              & {86.7\ms{0.80}} / {86.2\ms{0.82}}
		              & {68.3\ms{0.47}} / {62.2\ms{1.21}}
		              & {66.7\ms{0.25}} / {58.8\ms{0.42}}~$\arrvline$
		              & {72.9\ms{0.24}} / {71.0\ms{0.32}}
		              \\              
		              &     &   
		              & (-77.2\% / -84.4\%) 
		              & (-11.8\% / -27.0\%) 
		              & (-3.62\% / -15.7\%) \hspace{-0.095in} $\arrvline$ 
		              & (-48.0\% / -63.6\%) 
		              \\   
		ReMixMatch \cite{berthelot2019remixmatch}   &  \checkmark & - 
		              & {48.3\ms{0.14}} / {19.5\ms{0.85}}
		              & {75.1\ms{0.43}} / {71.9\ms{0.77}}
		              & {72.5\ms{0.10}} / {68.2\ms{0.32}}~$\arrvline$
		              & {49.0\ms{0.55}} / {17.1\ms{1.48}}
		              \\
		ReMixMatch$^{*}$    &  \checkmark & - 
		              & {85.0\ms{1.35}} / {84.3\ms{1.55}}
		              & {77.0\ms{0.12}} / {74.7\ms{0.04}}
		              & {72.8\ms{0.10}} / {68.8\ms{0.21}}~$\arrvline$
		              & {75.3\ms{0.03}} / {72.3\ms{0.04}}
		              \\
		\rowcolor{Gray} ReMixMatch$^{*}$ + DARP  &  \checkmark & - 
		              & {\textbf{89.7}\ms{0.15}} / {\textbf{89.4}\ms{0.17}}
		              & {\textbf{77.4}\ms{0.22}} / {75.0\ms{0.25}} 
		              & {\textbf{73.2}\ms{0.11}} / {69.2\ms{0.31}}~$\arrvline$
		              & {\textbf{80.1}\ms{0.11}} / {\textbf{78.5}\ms{0.17}}
		              \\              
		              &     &   
		              & (-31.4\% / -32.5\%) 
		              & (-1.72\% / -1.49\%) 
		              & (-1.53\% / -2.64\%) \hspace{-0.095in} $\arrvline$ 
		              & (-19.5\% / -22.5\%) 
		              \\	              
		FixMatch \cite{sohn2020fixmatch}     &  \checkmark & - 
		              & {68.9\ms{1.95}} / {42.8\ms{8.11}}
		              & {73.9\ms{0.25}} / {70.5\ms{0.52}}
		              & {69.6\ms{0.60}} / {62.6\ms{1.11}}~$\arrvline$ 
		              & {65.5\ms{0.05}} / {26.0\ms{0.44}}
		               \\
		              \rowcolor{Gray} FixMatch + DARP  &  \checkmark & - 
		              & {85.4\ms{0.55}} / {85.0\ms{0.65}}
		              & {{77.3}\ms{0.17}} / {\textbf{75.5}\ms{0.21}}
		              & 
		              {{72.9}\ms{0.24}} / {\textbf{69.5}\ms{0.18}}~$\arrvline$
		              & {74.9\ms{0.51}} / {72.3\ms{1.13}}
		              \\              
		              &     &   
		              & (-53.1\% / -73.8\%) 
		              & (-13.3\% / -17.0\%) 
		              & (-10.9\% / -18.4\%) \hspace{-0.095in} $\arrvline$ 
		              & (-31.3\% / -60.3\%) 
		              \\	             \bottomrule
	\end{tabular}
	\end{adjustbox}
    \end{center}
    \vspace{-0.15in}
\end{table*}

==> Imbalanced Semi-supervised Learning Arxiv (3)/table/Table3.tex <==
\begin{table}[t]
	\begin{center}
	\caption{Comparison of classification performance (bACC/GM) on CIFAR-10 across different distribution matching methods applied to ReMixMatch \cite{berthelot2019remixmatch} under $\gamma_l=100$.
    }
    \vspace{0.1in}
	\label{table:matching}
    \begin{adjustbox}{width=0.7\linewidth}
	\begin{tabular}{ccccc}
		\toprule
	    {Algorithm}        &  $\gamma_{u}=1$  & $\gamma_{u}= 50$ & $\gamma_{u}=100$ & $\gamma_{u}=100 ~(\text{reversed})$  \\ \midrule
		\cite{arazo2019pseudo} 
		& {81.4} / {80.5}
		& {76.0} / {72.7}
		& {72.5} / {67.8}~$\arrvline$   
		& {72.9} / {67.1} \\ 
		\cite{berthelot2019remixmatch} 
		& {85.0} / {84.3}
		& {77.0} / {74.7}
		& {73.8} / {69.5}~$\arrvline$
		& {75.3} / {72.3} \\ \midrule 
		DARP 
		& {\textbf{89.7}} / {\textbf{89.4}} 
		& {\textbf{77.4}} / {\textbf{75.0}} 
		& {\textbf{75.8}} / {\textbf{72.6}}~$\arrvline$ 
		& {\textbf{80.1}} / {\textbf{78.5}} \\ \bottomrule 
	\end{tabular}
    \end{adjustbox}
    \end{center}
    \vspace{-0.2in}
\end{table}

==> Imbalanced Semi-supervised Learning Arxiv (3)/table/Table4.tex <==
\begin{table*}[t]
	\begin{center}
	\caption{{Comparison of classification performance (bACC/GM) on CIFAR-100 and STL-10 under two different class-imbalance ratio $\gamma_l$. SSL denotes semi-supervised learning and RB denotes re-balancing. The numbers in brackets below the gray rows are relative test error gains from DARP, compared to applied baseline SSL algorithms, respectively. The best results are indicated in bold.}
    }
	\label{table:supple_other}
    \begin{adjustbox}{width=1.0\linewidth}
	\begin{tabular}{ccccccc}
		\toprule
		\multicolumn{3}{c}{}   & \multicolumn{2}{c}{CIFAR-100 ($\gamma_l= \gamma_u$)} & \multicolumn{2}{c}{STL-10 ($\gamma_l\neq \gamma_u$)} \\
        \cmidrule(r){4-5} \cmidrule(r){6-7}
        \vspace{0.15in}
		\multirow{2}{*}{Algorithm}       &
		\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} SSL \end{tabular}} &   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} RB \end{tabular}}
		              & \multirow{2}{*}{$\gamma_l=10$}  
		              & \multirow{2}{*}{$\gamma_l=20$}
		              & \multirow{2}{*}{$\gamma_l=10$}  
		              & \multirow{2}{*}{$\gamma_l=20$}
		              \\ \midrule
		Vanilla       & - & - 
		              & {55.9\ms{0.12}} / {50.7\ms{0.12}} 
		              & {49.5\ms{0.03}} / {40.3\ms{0.04}} 
		              & {56.4\ms{1.50}} / {51.8\ms{1.67}} 
		              & {48.1\ms{0.26}} / {38.2\ms{0.67}} 
		               \\\midrule 
	    Re-sampling   & - & \checkmark  
		              & {54.6\ms{0.05}} / {48.9\ms{0.40}}
		              & {48.1\ms{0.17}} / {38.3\ms{0.82}}
		              & {57.8\ms{0.76}} / {53.6\ms{0.80}} 
		              & {47.4\ms{0.16}} / {35.8\ms{0.11}} 
		              \\ 
	    LDAM-DRW      & - & \checkmark 
		              & {55.7\ms{0.75}} / {51.6\ms{0.08}}
		              & {50.4\ms{0.32}} / {45.4\ms{0.98}} 
		              & {58.0\ms{0.53}} / {54.4\ms{0.84}} 
		              & {50.2\ms{0.05}} / {42.4\ms{0.08}} 
		              \\ 
		cRT           & - & \checkmark  
		              & {56.2\ms{0.36}} / {52.2\ms{0.38}} 
		              & {50.7\ms{0.11}} / {43.8\ms{0.04}} 
		              & {59.2\ms{0.53}} / {55.7\ms{0.65}} 
		              & {49.2\ms{0.29}} / {42.3\ms{0.20}} 
		               \\ \midrule
		VAT           &  \checkmark & -  
		              & {54.6\ms{0.06}} / {48.6\ms{0.11}} 
		              & {48.5\ms{0.16}} / {38.5\ms{0.25}} 
		              & {64.2\ms{0.33}} / {61.1\ms{0.50}} 
		              & {56.2\ms{0.03}} / {50.5\ms{0.08}} 
		               \\ 
		Mean-Teacher  &  \checkmark & -  
		              & {54.1\ms{0.13}} / {48.2\ms{0.05}} 
		              & {48.2\ms{0.13}} / {37.6\ms{0.07}} 
		              & {57.7\ms{0.10}} / {54.8\ms{0.87}} 
		              & {48.0\ms{0.47}} / {35.3\ms{3.81}} 
		               \\ 
		MixMatch      &  \checkmark & - 
		              & {60.1\ms{0.39}} / {48.1\ms{4.08}}
		              & {53.4\ms{0.04}} / {41.9\ms{0.16}}
		              & {56.3\ms{0.46}} / {48.2\ms{1.08}} 
		              & {45.2\ms{0.19}} / {22.0\ms{0.12}} 
		                \\
	\rowcolor{Gray}	 MixMatch + DARP             
	                  & \checkmark & - 
		              & {60.9\ms{0.24}} / {55.8\ms{0.05}}
		              & {54.8\ms{0.27}} / {45.6\ms{0.48}}
		              & {67.9\ms{0.24}} / {65.1\ms{0.51}} 
		              & {58.3\ms{0.73}} / {52.2\ms{1.01}}  
		              \\
		              & &   
		              & (-2.04\% / -14.8\%) 
		              & (-3.38\% / -6.33\%) 
		              & (-26.7\% / -32.7\%) 
		              & (-23.9\% / -38.8\%) 
		              \\
	    ReMixMatch    & \checkmark & - 
		              & {59.2\ms{0.03}} / {52.1\ms{0.13}} 
		              & {53.5\ms{0.03}} / {42.3\ms{0.13}} 
		              & {67.8\ms{0.45}} / {61.1\ms{0.92}} 
		              & {60.1\ms{1.18}} / {44.9\ms{1.52}} 
		               \\
	\rowcolor{Gray} ReMixMatch + DARP
	                  & \checkmark & -
		              & {{59.8}\ms{0.20}} / {{52.9}\ms{0.41}}  
		              & {{54.4}\ms{0.07}} / {{44.2}\ms{0.07}} 
		              & {\textbf{79.4}\ms{0.07}} / {\textbf{78.2}\ms{0.10}} 
		              & {\textbf{70.9}\ms{0.44}} / {\textbf{67.0}\ms{1.62}}  \\ 
		              & &   
		              & (-1.25\% / -1.59\%) 
		              & (-1.88\% / -3.23\%) 
		              & (-36.0\% / -44.0\%) 
		              & (-27.0\% / -40.0\%)
		               \\
		FixMatch      &  \checkmark & - 
		              & {60.1\ms{0.05}} / {54.4\ms{0.11}}
		              & {54.0\ms{0.04}} / {44.4\ms{0.17}}
		              & {72.9\ms{0.09}} / {69.6\ms{0.01}} 
		              & {63.4\ms{0.21}} / {52.6\ms{0.09}} 
		               \\
	\rowcolor{Gray} FixMatch + DARP
	                  & \checkmark & - 
		              & {\textbf{61.1}\ms{0.23}} / {\textbf{56.4}\ms{0.28}}
		              & {\textbf{54.9}\ms{0.05}} / {\textbf{46.4}\ms{0.41}}
		              & {77.8\ms{0.33}} / {76.5\ms{0.40}} 
		              & {69.9\ms{1.77}} / {65.4\ms{3.07}}  
		              \\ 
		              & &   
		              & (-2.55\% / -4.40\%) 
		              & (-1.97\% / -3.60\%) 
		              & (-18.2\% / -22.8\%) 
		              & (-17.9\% / -27.0\%)
		               \\\bottomrule
	\end{tabular}
    \end{adjustbox}
    \end{center}
    \vspace{-0.15in}
\end{table*}

==> Imbalanced Semi-supervised Learning Arxiv (3)/table/Table5.tex <==
\begin{table*}[h]
    \begin{center}
	\caption{Comparison of classification performance (bACC/GM) on SUN397. SSL denotes semi-supervised learning and RB denotes re-balancing. The numbers in brackets below the gray rows are relative test error gains from DARP, compared to applied baseline SSL algorithms, respectively. The best results are indicated in bold.
    }
	\label{table:sun-397}
	\vspace{0.05in}
    \begin{adjustbox}{width=0.5\linewidth}
	\begin{tabular}{cccc}
		\toprule
	    Method          & SSL & RB &  $\gamma \approx 46$   \\ \midrule
	    Vanilla         & - & - &  {38.3\ms{0.05}} / {29.9\ms{0.08}} \\
	    cRT             & - & \checkmark &  {39.3\ms{0.21}} / {33.7\ms{0.37}} \\
		FixMatch        & \checkmark & - &  {44.9\ms{0.11}} / {35.7\ms{0.66}}  \\ 
		\rowcolor{Gray} FixMatch + DARP & \checkmark & - &  {\textbf{45.5}\ms{0.32}} / {\textbf{37.5}\ms{0.04}} \\ 
		&&& (-1.09\% / -2.80\%) \\ \bottomrule 
	\end{tabular}
    \end{adjustbox}
    \end{center}
\end{table*}

==> Imbalanced Semi-supervised Learning Arxiv (3)/table/Table6.tex <==
\begin{table*}[h]
	\begin{center}
	\caption{Comparison of classification performance (bACC/GM) on CIFAR-10 under three different class-imbalance ratio $\gamma=\gamma_l=\gamma_u$. SSL denotes semi-supervised learning and RB denotes re-balancing. The numbers in brackets below the gray rows are relative test error gains from DARP, compared to applied baseline SSL algorithms, respectively. The best results are indicated in bold.
    }
	\label{table:cifar_crt}
	\vspace{0.05in}
    \begin{adjustbox}{width=0.9\linewidth}
	\begin{tabular}{cccccc}
		\toprule
		\multicolumn{3}{c}{}   & \multicolumn{3}{c}{CIFAR-10} \\
        \cmidrule(r){4-6}
        \vspace{0.15in}
		\multirow{2}{*}{Algorithm}       &
		\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} SSL \end{tabular}} &   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} RB \end{tabular}}
		              & \multirow{2}{*}{$\gamma=50$}  
		              & \multirow{2}{*}{$\gamma=100$}
		              & \multirow{2}{*}{$\gamma=150$} \\ \midrule
		Vanilla       & - & - 
		              & {65.2\ms{0.05}} / {61.1\ms{0.09}} 
		              & {58.8\ms{0.13}} / {51.0\ms{0.11}} 
		              & {55.6\ms{0.43}} / {44.0\ms{0.98}} 
		               \\\midrule 
	    ReMixMatch \cite{berthelot2019remixmatch}   
	                  & \checkmark & - 
		              & {81.5\ms{0.26}} / {80.2\ms{0.32}} 
		              & {73.8\ms{0.38}} / {69.5\ms{0.84}} 
		              & {69.9\ms{0.47}} / {62.5\ms{0.35}}
		               \\
	    \rowcolor{Gray} ReMixMatch + DARP
	                  & \checkmark & -
		              & {82.1\ms{0.14}} / {{80.8}\ms{0.09}}  
		              & {75.8\ms{0.09}} / {{72.6}\ms{0.24}} 
		              & {71.0\ms{0.27}} / {{64.5}\ms{0.68}} \\ 
		              & &   
		              & (-3.45\% / -3.52\%) 
		              & (-7.84\% / -10.2\%) 
		              & (-3.60\% / -5.19\%)  
		               \\ \midrule
		ReMixMatch + cRT   
	                  & \checkmark & \checkmark 
		              & {86.8\ms{0.50}} / {86.5\ms{0.49}} 
		              & {81.4\ms{0.41}} / {80.7\ms{0.45}} 
		              & {78.9\ms{0.84}} / {77.8\ms{0.94}}
		               \\
	    \rowcolor{Gray} ReMixMatch + DARP + cRT 
	                  & \checkmark & \checkmark
		              & {\textbf{87.3}\ms{0.16}} / {\textbf{87.0}\ms{0.11}}  
		              & {\textbf{83.5}\ms{0.07}} / {\textbf{83.1}\ms{0.09}} 
		              & {\textbf{79.7}\ms{0.54}} / {\textbf{78.9}\ms{0.49}} \\ 
		              & &   
		              & (-4.33\% / -3.63\%) 
		              & (-11.3\% / -12.2\%) 
		              & (-3.61\% / -5.12\%)  
		               \\ \bottomrule
	\end{tabular}
    \end{adjustbox}
    \end{center}
\end{table*}
